How to Overcome Curse-of-Dimensionality for Out-of-Distribution Detection?

Machine learning models deployed in the wild can be challenged by out-of-distribution (OOD) data from unknown classes. Recent advances in OOD detection rely on distance measures to distinguish samples that are relatively far away from the in-distribution (ID) data. Despite the promise, distance-based methods can suffer from the curse-of-dimensionality problem, which limits the efficacy in high-dimensional feature space. To combat this problem, we propose a novel framework, Subspace Nearest Neighbor (SNN), for OOD detection. In training, our method regularizes the model and its feature representation by leveraging the most relevant subset of dimensions (i.e. subspace). Subspace learning yields highly distinguishable distance measures between ID and OOD data. We provide comprehensive experiments and ablations to validate the efficacy of SNN. Compared to the current best distance-based method, SNN reduces the average FPR95 by 15.96% on the CIFAR-100 benchmark.

==> macros-includes.tex <==
\usepackage{multirow,epsfig,pdflscape,graphicx,amsmath,amssymb}
\usepackage[table,x11names]{xcolor}
\usepackage{float}
\usepackage{mathrsfs}
\usepackage{empheq}
\usepackage{rotating}
\usepackage{boldline}
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
%\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{lipsum}
%\usepackage[noadjust]{cite}
\usepackage{array, tabularx,  ragged2e,  booktabs}
%\usepackage[font=small,skip=5pt,belowskip=0pt]{caption}
%\setlength{\textfloatsep}{5pt}
\usepackage{longtable}
%\usepackage{textcomp}
%\usepackage{siunitx}
%\usepackage{subfig}
\usepackage{array}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
%\usepackage{algorithm} % http://ctan.org/pkg/algorithms
\usepackage[noend]{algpseudocode} % http://ctan.org/pkg/algorithmicx

\usepackage{algpseudocode}
\usepackage{romannum}
%\usepackage{amsthm}
\usepackage{graphicx}
%\usepackage{xcolor}

\usepackage{algorithmicx}

%\usepackage[usenames,dvipsnames]{xcolor}
%\usepackage{times}
\usepackage{epsfig}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{appendix}
%\usepackage{etoolbox}
%\usepackage{soul}
\usepackage{tabularx}
\usepackage{rotating,comment}
%\usepackage[outercaption]{sidecap}  
%\usepackage{wrapfig}
%\renewcommand{\restriction}{\mathord{\upharpoonright}}

% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

%\usepackage[inline]{enumitem}

%\newcommand\figref[1]{Figure~\ref{#1}}
%\newcommand\tabref[1]{Table~\ref{#1}}

%\usepackage{hyperref}

% \BeforeBeginEnvironment{appendices}{\clearpage}

% \newcolumntype{Y}{>{\centering\arraybackslash}X}
% \def\lce{{\mathcal{L}_{\rm CE}}}
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\minimize}{minimize}

% \definecolor{todocolor}{RGB}{200,120,120}
% \sethlcolor{todocolor}
% \newcommand{\todo}[1]{\textcolor{black}{\hl{#1}}}

%\newcommand{\figref}[1]{Fig.~\ref{#1}}
%\newcommand{\secref}[1]{Sec.~\ref{#1}}
%\usepackage{graphicx} 
%\usepackage[showframe]{geometry}
% \usepackage{array}
% \newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
% \newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
% \def\X{{\mathcal{X}}}
% \def\Y{{\mathcal{Y}}}
% \def\D{{\mathcal{D}}}

% \def\dP{{\mathbb{P}}}
% \def\cP{{\mathcal{P}}}
% \def\cQ{{\mathcal{Q}}}
% \def\cM{{\mathcal{M}}}

% \def\real{{\mathbb{R}}}

% \def\ood{\textsc{ood}\xspace}
% \def\iid{\textsc{iid}\xspace}
% \def\id{\textsc{id}\xspace}
% \def\sota{\textsc{sota}\xspace}
% \def\dnn{\textsc{dnn}\xspace}

% \def\xt{{\Tilde{x}}}
% \def\yt{{\Tilde{y}}}
% \def\hbe{{\mathbf{\emph{h}}}}
% \def\HC{{\mathcal{H}}}

% \newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
% \newcolumntype{N}{@{}m{0pt}@{}@{}}

% \newcommand{\myfirstpara}[1]{\noindent \textbf{#1:}}
% \newcommand{\mypara}[1]{\vspace{0.2em} \myfirstpara{#1}}

% \newcommand{\multilineC}[1]{\begin{tabular}[b]{@{}c@{}}#1\end{tabular}}
% \newcommand{\multilineCB}[1]{\textbf{\multilineC{#1}}}
% \newcommand{\vertext}[1]{\begin{turn}{90} {#1} \end{turn}}

% %\fboxsep=0.2mm%padding thickness
% %\fboxrule=0.02pt%border thickness

% \graphicspath{{images/}}
% \graphicspath{{./imgs/}}
% \usepackage{titlesec}
% \usepackage{lipsum}% just to generate text for the example

% \titlespacing*{\section}
% {0pt}{4ex}{4ex}
% \titlespacing*{\subsection}
% {0pt}{3ex}{3ex}


==> sections/calibration.tex <==
\subsection{Model Calibration}
\label{subsec:calibration}

\input{tables/calibration_main}

Beyond\ood detection tasks, in this section we show that our subspace training algorithm also leads to a significant improvement in model calibration. 

\paragraph{Datasets.} We train on three common benchmark datasets: CIFAR-10/100~\cite{krizhevsky2009learning} and Tiny-ImageNet\cite{deng2009imagenet} (200 classes). For each dataset, we have a separate train and test set. We further split the train set into two mutually exclusive sets: (1) $90\%$ of the train samples are used for training the model, and (2) the remaining $10\%$ of samples are used for validation and hyper-parameter adjustment for post-hoc calibration.

\paragraph{Evaluation Metrics.} To measure model calibration we report: (1) \textbf{Expected Calibration Error (ECE)}~\cite{naeini2015obtaining}: is the weighted average of differences in confidence of predicted class and accuracy of samples predicted with particular confidence. (2) \textbf{Static Calibration Error (SCE)}~\cite{nixon2019measuring}: is a simple class-wise extension of ECE. Refer Appendix for a detailed overview of the metrics used. 


\paragraph{Learning subspace improves calibration.} In Table~\ref{tab:calibration_1}, we observe that our subspace-based training algorithm improves calibration performance. In particular, we consider three losses that are commonly studied for calibration: (1) Cross Entropy Loss (NLL), (2) Label Smoothing (LS)~\cite{muller2019does}, and (3) Focal Loss (FL)~\cite{lin2017focal}. We train the model with each of these losses and measure calibration performance with and without subspace regularization. For clarity, we refer to the technique using our subspace-based learning as ``\textbf{ * + Subspace }'', where * refers to NLL/FL/LS. We see from Table~\ref{tab:calibration_1} that across multiple datasets, using subspace improves the calibration performance of all the loss functions. Specifically, we note that FL+Subspace gives the best performance on multiple datasets. In the Appendix\SL{???}, we further study the effect of combining different post-hoc calibration methods, namely Temperature Scaling and Dirichlet Calibration, over various calibration strategies studied in Table~\ref{tab:calibration_1}.


==> tables/calibration_posthoc.tex <==
\newcolumntype{?}{!{\vrule width 1pt}}
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llcccc}
\toprule
\multirow{2}{1.75cm}{\textbf{Method}} &  
\multirow{2}{1.5cm}{\textbf{Post-Hoc}}
& \multicolumn{2}{c}{\textbf{CIFAR-10}} & \multicolumn{2}{c}{\textbf{CIFAR-100}} \\

\cmidrule{3-6}
& & SCE & ECE & SCE & ECE \\
\midrule
\multirow{2}{*}{NLL} & None & 11.5 & 5.6 & 3.7 & 15.1 \\
& TS & 3.9 & 1.4 & 1.9 & 2.3\\
\midrule
\multirow{2}{*}{NLL (w. Subspace)} & None & 9.6 & 4.4 & 2.5 & 5.8 \\
 & \rowcolor{COLOR_ZS} TS & \textbf{4.2} & \textbf{1.1} & \textbf{1.9} & \textbf{2.3}\\

\bottomrule

\end{tabular}}
\caption{Post-hoc Calibration Performance of \name using Temperature Scaling. Model used is ResNet 50.}
\label{tab:calibration_post_hoc}
\end{table}



==> tables/hard_ood_compress.tex <==
\newcolumntype{?}{!{\vrule width 1pt}}
\begin{table}[t]
\centering
\small
\begin{tabular}{lcccc}
\multirow{2}{1.5cm}{\textbf{Methods}} & \multicolumn{2}{c}{\textbf{Far-OOD}} & \multicolumn{2}{c}{\textbf{Near-OOD}}\\
\cmidrule{2-5}
& \textbf{FPR95}  & \textbf{AUROC} & \textbf{FPR95}  & \textbf{AUROC}\\
& \downarrow & \uparrow & \downarrow & \uparrow \\
\toprule
\emph{Methods using model outputs}\\
MSP~\cite{hendrycks2016baseline} & 52.11 & 91.79 & 64.66 & 85.28 \\
ODIN~\cite{liang2018enhancing}  & 26.47 & 94.48 & 52.32 & 88.90\\
GODIN~\cite{hsu2020generalized}  & 17.42  & 95.84 & 60.69 & 82.37 \\
Energy score~\cite{liu2020energy}  & 28.40 & 94.22 & 50.64 & 88.66 \\
LogitNorm~\cite{wei2022mitigating}  & 19.61 & 95.51 & 55.08 & 88.03\\
DICE~\cite{sun2022dice}  & 20.83 & 95.24 & 58.60 & 87.11 \\
\midrule
\emph{Methods using feature representatins}\\
Mahalanobis~\cite{lee2018simple} & 44.55 & 82.56 & 87.71 & 78.93 \\
KNN~\cite{sun2022knn}  & 18.50 & 96.36 & 58.34 & 87.90 \\
\midrule 
\rowcolor{COLOR_ZS} \name (ours) & \textbf{14.47} & \textbf{97.20}  & \textbf{49.54} &  \textbf{90.05}\\
 & $\pm{0.87}$ & $\pm{0.27}$ & $\pm{1.09}$ & $\pm{0.65}$\\
\bottomrule
\end{tabular}
\caption{Performance comparison on near-OOD and far-OOD detection task. Architecture used is DenseNet-101 and ID is CIFAR-10. Best performing results are marked in \textbf{bold}. We report the mean and variance across 3 different training runs. }
\label{tab:hard_ood}
\end{table}



==> tables/imagenet.tex <==
\newcolumntype{?}{!{\vrule width 1pt}}
\begin{table*}[t]

\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l*{11}c}
\toprule
\multirow{2}{1.5cm}{\textbf{Methods}} & \multicolumn{8}{c}{\textbf{OOD Datasets}} & \multicolumn{2}{c}{\multirow{2}{*}{\centering\textbf{Average}}} & \textbf{ID Acc.}\\

\cmidrule{2-9}

& \multicolumn{2}{c}{\textbf{iNaturalist}} & \multicolumn{2}{c}{\textbf{SUN}} & \multicolumn{2}{c}{\textbf{Places}} & \multicolumn{2}{c}{\textbf{Textures}} & &  \\

 & FPR95 & AUROC & FPR95 & AUROC & FPR95 & AUROC &  FPR95 & AUROC & FPR95 & AUROC \\
& $\pmb{\downarrow}$ & $\pmb{\uparrow}$  & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ &  $\pmb{\uparrow}$ & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\uparrow}$  \\
 \midrule
 \multicolumn{12}{c}{\textbf{Without Sparsification}} \\
MSP & 54.99 & 87.74 & 70.83 & 80.86 & 73.99 & 79.76 & 68.00 & 79.61 & 66.95 & 81.99 & 75.75\\
ODIN & 47.66 & 89.66 & 60.15 & 84.59 & 67.89 & 81.78 & 50.23 & 85.62 & 56.48 & 85.41 & 75.75 \\
GODIN & 61.91 & 85.40 & 60.83 & 85.60 & 63.70 & 83.81 & 77.86 & 73.27 & 66.07 & 82.02 & 70.43\\
Mahalanobis & 97.00 & 52.65 & 98.50 & 42.41 & 98.40 & 41.79 & 55.80 & 85.01 & 87.43 & 55.47 & 75.75\\
Energy & 55.72 & 89.95 & 59.26 & 85.89 & 64.92 & 82.86 & 53.72 & 85.99 & 58.41 & 86.17 & 75.75 \\
KNN & 59.00 & 86.47 & 68.82 & 80.72 & 76.28 & 75.76 & 11.77 & 97.07 & 53.97 & 85.01 & 75.75\\
\midrule
 \multicolumn{12}{c}{\textbf{With Sparsification}} \\
ReAct & 24.38 & 95.41 & 27.20 & 93.89 & 39.54 & 90.12 & 48.56 & 88.54 & 34.92 & 91.99 & 73.67 \\
DICE & 25.63 & 94.49 & 35.15 & 90.83 & 46.49 & 87.48 & 31.72 & 90.30 & 34.75 & 90.77 & 73.58 \\
\rowcolor{Gray} DICE (w/KNN) & 81.06 & 78.24 & 84.00 & 74.18 & 87.55 & 70.57 & 37.98 & 91.54 & 72.65 & 78.64 & 73.58 \\
SPARTAN (w/KNN) & 72.91 & 82.64 & 83.13 & 74.82 & 88.21 & 69.53 & 14.50 & 96.63 & 64.11 & 82.04 & 76.04 \\
SPARTAN (w/Energy) & 26.04 & 94.91 & 31.98 & 90.42 & 40.41 & 90.32 & 34.73 & 90.42 & \textbf{33.29} & \textbf{92.06} & \textbf{76.04} \\

\bottomrule

\end{tabular}%
}
\caption{\small \textbf{Results on ImageNet.} Comparison with competitive out-of-distribution detection method on ImageNet dataset. All values are percentages. $\pmb{\downarrow}$ indicates smaller values are better and $\pmb{\uparrow}$ indicates larger values are better. Best performing results are marked in \textbf{bold}.}
\label{tab:ood_imagenet}
\end{table*}



==> tables/new_tab.tex <==
\begin{table}[t]
\parbox{0.48\columnwidth}{
\caption{\small Performance comparison on CIFAR-100 dataset. Architecture is DenseNet-101.  Best  results are in \textbf{bold}. We report the mean and variance across 3 different training runs.}
\label{tab:cifar-100}
\small
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\textbf{Method} & \textbf{FPR95}  & \textbf{AUROC} & \textbf{ID Acc.}\\
& \downarrow & \uparrow & \uparrow \\
\toprule
\emph{Methods using model outputs}\\
MSP~\cite{hendrycks2016baseline} & 77.59 & 76.47 &  75.14\\
ODIN~\cite{liang2018enhancing} & 56.39 & 86.02 & 75.14\\
GODIN~\cite{hsu2020generalized} & 44.08 &  89.05 & 74.37\\
Energy score~\cite{liu2020energy} & 57.07 &  84.83 &  75.14\\
LogitNorm~\cite{wei2022mitigating} & 61.10 & 84.72 & 75.42\\
DICE~\cite{sun2022dice} & 49.72 & 87.23 & 68.65 \\
\midrule 
\emph{Methods using feature representations}\\
Mahalanobis~\cite{lee2018simple} & 56.93 & 80.27 &  75.14\\
KNN~\cite{sun2022knn} & 47.21 & 85.27 & 75.14\\
\midrule 
\rowcolor{COLOR_ZS} \name (ours) & \textbf{31.25} &  \textbf{90.76} & \textbf{75.59}\\
& $\pm{1.25}$ & $\pm{0.36}$ & $\pm{0.08}$\\
\bottomrule
\end{tabular}}}
\hfill
\parbox{0.48\columnwidth}{
\caption{\small Performance comparison on near-OOD and far-OOD detection task. Architecture used is DenseNet-101 and ID is CIFAR-10. Best performing results are marked in \textbf{bold}. We report the mean and variance across 3 different training runs. }
\label{tab:hard_ood}
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\multirow{2}{1.5cm}{\textbf{Methods}} & \multicolumn{2}{c}{\textbf{Far-OOD}} & \multicolumn{2}{c}{\textbf{Near-OOD}}\\
\cmidrule{2-5}
& \textbf{FPR95}  & \textbf{AUROC} & \textbf{FPR95}  & \textbf{AUROC}\\
& \downarrow & \uparrow & \downarrow & \uparrow \\
\toprule
\emph{Methods using model outputs}\\
MSP~\cite{hendrycks2016baseline} & 52.11 & 91.79 & 64.66 & 85.28 \\
ODIN~\cite{liang2018enhancing}  & 26.47 & 94.48 & 52.32 & 88.90\\
GODIN~\cite{hsu2020generalized}  & 17.42  & 95.84 & 60.69 & 82.37 \\
Energy score~\cite{liu2020energy}  & 28.40 & 94.22 & 50.64 & 88.66 \\
LogitNorm~\cite{wei2022mitigating}  & 19.61 & 95.51 & 55.08 & 88.03\\
DICE~\cite{sun2022dice}  & 20.83 & 95.24 & 58.60 & 87.11 \\
\midrule
\emph{Methods using feature representatins}\\
Mahalanobis~\cite{lee2018simple} & 44.55 & 82.56 & 87.71 & 78.93 \\
KNN~\cite{sun2022knn}  & 18.50 & 96.36 & 58.34 & 87.90 \\
\midrule 
\rowcolor{COLOR_ZS} \name (ours) & \textbf{14.47} & \textbf{97.20}  & \textbf{49.54} &  \textbf{90.05}\\
 & $\pm{0.87}$ & $\pm{0.27}$ & $\pm{1.09}$ & $\pm{0.65}$\\
\bottomrule
\end{tabular}}}
\end{table}

==> tables/new_tab_1.tex <==
\begin{table}[b]
\small
\centering
\captionof{table}{\small Performance comparison on CIFAR-100 dataset. We use DenseNet-101 for all baselines. Best  results are in \textbf{bold}. We report the mean and variance across 3 different training runs.}
\label{tab:cifar-100}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccc}
\textbf{Method} & \textbf{FPR95}  & \textbf{AUROC} & \textbf{ID Acc.}\\
& $\downarrow$ & $\uparrow$ & $\uparrow$ \\
\toprule
\emph{Methods using model outputs}\\
MSP~\cite{hendrycks2016baseline} & 77.59 & 76.47 &  75.14\\
ODIN~\cite{liang2018enhancing} & 56.39 & 86.02 & 75.14\\
GODIN~\cite{hsu2020generalized} & 44.08 &  89.05 & 74.37\\
Energy score~\cite{liu2020energy} & 57.07 &  84.83 &  75.14\\
ReAct~\cite{sun2021react} & 75.06 & 79.51 & 66.56\\
GradNorm~\cite{huang2021importance} & 63.05 & 79.80 & 75.14\\
LogitNorm~\cite{wei2022mitigating} & 61.10 & 84.72 & 75.42\\
DICE~\cite{sun2022dice} & 49.72 & 87.23 & 68.65 \\
\midrule 
\emph{Methods using feature representations}\\
Mahalanobis~\cite{lee2018simple} & 56.93 & 80.27 &  75.14\\
KNN~\cite{sun2022knn} & 47.21 & 85.27 & 75.14\\
\midrule 
 \name (ours) & \textbf{31.25} & \textbf{90.76} & \textbf{75.59}\\
& $\pm{1.25}$ & $\pm{0.36}$ & $\pm{0.08}$\\
\bottomrule
\end{tabular}}

\quad
\begin{minipage}[t]{0.46\textwidth}%
\centering
\small
\captionof{table}{\small Performance comparison on near-OOD and far-OOD detection task. Architecture used is DenseNet-101 and ID data is CIFAR-10. We report the mean and variance across 3 training runs. }
\label{tab:hard_ood}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccc}
\multirow{2}{1.5cm}{\textbf{Methods}} & \multicolumn{2}{c}{\textbf{Far-OOD}} & \multicolumn{2}{c}{\textbf{Near-OOD}}\\
\cmidrule{2-5}
& \textbf{FPR95}  & \textbf{AUROC} & \textbf{FPR95}  & \textbf{AUROC}\\
& $\downarrow$ & $\uparrow$ & $\downarrow$ & $\uparrow$ \\
\toprule
\emph{Using model outputs}\\
MSP~\cite{hendrycks2016baseline} & 52.11 & 91.79 & 64.66 & 85.28 \\
ODIN~\cite{liang2018enhancing}  & 26.47 & 94.48 & 52.32 & 88.90\\
GODIN~\cite{hsu2020generalized}  & 17.42  & 95.84 & 60.69 & 82.37 \\
Energy score~\cite{liu2020energy}  & 28.40 & 94.22 & 50.64 & 88.66 \\
\cite{sun2021react} & 82.84 & 76.32 & 79.97 & 77.16\\
ReAct~\cite{sun2021react} & 33.12 & 94.32 & 53.51 & 88.96\\
GradNorm~\cite{huang2021importance} & 24.79 & 92.58 & 65.44 & 79.31\\
LogitNorm~\cite{wei2022mitigating}  & 19.61 & 95.51 & 55.08 & 88.03\\
DICE~\cite{sun2022dice}  & 20.83 & 95.24 & 58.60 & 87.11 \\
\midrule
\emph{Using feature representations}\\
Mahalanobis~\cite{lee2018simple} & 44.55 & 82.56 & 87.71 & 78.93 \\
KNN~\cite{sun2022knn}  & 18.50 & 96.36 & 58.34 & 87.90 \\
\midrule 
 \name (ours) & \textbf{14.99} & \textbf{97.15}  & \textbf{50.10} &  \textbf{89.80}\\
 & $\pm{0.87}$ & $\pm{0.27}$ & $\pm{1.09}$ & $\pm{0.65}$\\
\bottomrule
\end{tabular}}
\end{minipage}%
\end{table}

==> tables/ood_main.tex <==
\newcolumntype{?}{!{\vrule width 1pt}}

\begin{table*}[t]

\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l*{6}c?*{6}c}
\toprule
\textbf{Model} & \multicolumn{6}{c?}{\centering
\textbf{DenseNet-101}} & \multicolumn{6}{c}{\centering \textbf{ResNet-50}} \\
\midrule

ID-Dataset & \multicolumn{3}{c}{\centering CIFAR-10} & \multicolumn{3}{c?}{\centering CIFAR-100} & \multicolumn{3}{c}{\centering CIFAR-10} & \multicolumn{3}{c}{\centering CIFAR-100} \\
\cmidrule{2-13}
 & FPR95 & AUROC & Acc. & FPR95 & AUROC & Acc. & FPR95 & AUROC & Acc. & FPR95 & AUROC & Acc.\\
& $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ & $\pmb{\uparrow}$  & $\pmb{\uparrow}$\\
 \midrule
& \multicolumn{12}{c}{\textbf{Without Sparsification}} \\
MSP & 49.95 & 92.05 & 94.15 & 79.10 & 75.39 & 75.08 & 66.94 & 87.25 & 92.83 & 84.02 & 72.83 & 72.66 \\
ODIN & 30.02 & 93.86 & 94.15 & 55.96 & 85.16 & 75.08 & 47.21 & 90.89 & 92.83 & 73.03 & 80.34 & 72.66\\
Mahalanobis & 35.88 & 87.56 & 94.15 & 74.57 & 66.03 & 75.08 & 56.78 & 85.65 & 92.83 & 76.84 & 68.12 &  72.66\\
GODIN & 28.98 & 92.48 & 94.22 & 55.38 & 83.76 & 74.50 & 45.36 & 91.85 & 92.56 & 63.21 & 82.98 & 73.85\\
Energy & 30.16 & 92.44 & 94.15 & 68.03 & 81.40 & 75.08 & 50.03 & 90.46 & 92.83 & 74.78 & 80.07 & 72.66  \\
LogitNorm & 19.61 & 95.51 & 93.94 & 61.10 & 84.72 & 75.42 & 43.51 & 92.53 & 92.13 & 68.01 & 81.50 & 74.71 \\
KNN & 17.02 & 95.82 & 94.15 & 50.62 & 81.35 & 75.08 & 38.14 & 93.23 & 92.83 & 60.97 & 75.70 & 72.66 \\
\midrule
& \multicolumn{12}{c}{\textbf{With Sparsification}} \\
ReAct & 26.45 & 94.95 & 93.58 & 62.27 & 84.47 & 72.56 & 35.87 & 91.65 & 91.48 & 62.71 & 83.65 & 70.60 \\
DICE & 20.83 & 95.24 & 92.11 & 49.72 & 87.23 & 68.65 & 48.41 & 90.14 & 91.23 & 68.94 & 80.22 & 65.67 \\
\midrule
SPARTAN w/ Energy & 15.28 & 96.51 & 94.34 & 40.33 & 89.15 & 76.12 & 27.30 & 95.15 & 93.60 & 51.50 & 88.05 & 75.89\\
SPARTAN w/ KNN & \textbf{15.10} & \textbf{97.10} & \textbf{94.34} & \textbf{29.14} & \textbf{90.94} & \textbf{76.12} & \textbf{23.19} & \textbf{95.15} & \textbf{93.60} & \textbf{40.30} & \textbf{88.08} & \textbf{75.89}\\
\midrule
SNN w/ MA & 16.91 & 96.66 & 94.50 & 32.81 & 90.11 & 75.33 & 16.52 & 96.88 & 93.60 & 43.50 & 87.08 & 75.4 \\ 
SNN w/Dyn-K & 21.28 & 95.83 & 94.22 & 35.52 & 89.77 & 75.83 & 22.06 & 95.84 & 93.85 &  48.74 & 84.94 & 76.1 \\

\bottomrule

\end{tabular}%
}
\caption{\small \textbf{Results on CIFAR-10/100.} Comparison with competitive out-of-distribution detection method on CIFAR benchmarks. All values are percentages and are averaged over 6 \ood test datasets. The full results for each dataset are provided in Appendix. Mean and standard deviation are estimated across 3 independent runs. $\pmb{\downarrow}$ indicates smaller values are better and $\pmb{\uparrow}$ indicates larger values are better. Best performing results are marked in \textbf{bold}. \soumya{Added the table just for easy reference for now.}}
\label{tab:ood_main}
\end{table*}




==> tables/ood_scoring.tex <==
\newcolumntype{?}{!{\vrule width 1pt}}
\begin{table*}[t]

\small
\centering
\scalebox{0.9}{
\begin{tabular}{lcc?cc?cc}
\toprule
\multirow{3}{*}{\textbf{Method}} & \multicolumn{2}{c}{\centering
\textbf{CIFAR-10}} & \multicolumn{2}{c}{\centering \textbf{CIFAR-100}} & \multicolumn{2}{c}{\centering \textbf{ImageNet}} \\

 & FPR95 & AUROC & FPR95 & AUROC & FPR95 & AUROC \\
& $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ &  $\pmb{\downarrow}$ & $\pmb{\uparrow}$ \\
 \midrule
MSP~\cite{hendrycks2016baseline} & 48.7 & 92.4 & 80.1 & 74.4 &66.95 & 81.99 \\
MSP + SPARTAN & 46.0 & 92.8 & 74.5 & 77.2 & 62.84 & 83.50\\
\midrule
ODIN~\cite{liang2018enhancing} & 24.7 & 93.7 & 58.1 & 84.5 & 56.48 & 85.41\\
ODIN + SPARTAN & 22.8 & 95.6 & 57.3 & 85.4 & 45.84 & 89.73\\
\midrule
Energy~\cite{liu2020energy} & 26.5 & 94.6 & 68.4 & 81.2 & 58.41 & 86.17 \\
Energy + SPARTAN & 15.4 & 96.5 & 40.3 & 89.2 & 33.29 & 92.06\\
\midrule
KNN~\cite{sun2022knn} & 17.1 & 95.8 & 50.6 & 81.3 & 53.97 & 85.01 \\
KNN + SPARTAN & \textbf{15.1} & \textbf{97.1} & \textbf{29.1} & \textbf{90.9} & 0 & 0 \\
\bottomrule
\end{tabular}}
\caption{\small SPARTAN is compatible with different \ood scoring functions. For each \id dataset, we use the same model and compare performance with and without SPARTAN respectively. All values are percentages and are average over multiple \ood datasets. Best performing results are marked in \textbf{bold}.}
\label{tab:ood_score}
\end{table*}



==> tables/open_ood_c10.tex <==
\begin{table}[t!]

\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l*{6}c|*{10}c}
 \multirow{2}{1.5cm}{\textbf{Methods}} & \multicolumn{6}{c|}{\textbf{Near OOD}} & \multicolumn{10}{c}{\textbf{Far OOD}} \\

\cmidrule{2-17}

& \multicolumn{2}{c}{\textbf{CIFAR-10}} & \multicolumn{2}{c}{\textbf{TIN}} & \multicolumn{2}{c|}{\textbf{Avg.}} &
\multicolumn{2}{c}{\textbf{MNIST}} &
\multicolumn{2}{c}{\textbf{SVHN}} & \multicolumn{2}{c}{\textbf{Textures}} & \multicolumn{2}{c}{\textbf{Places365}} & \multicolumn{2}{c}{\textbf{Avg.}} \\

& FPR95 & AUROC & FPR95 & AUROC & FPR95 & AUROC &  FPR95 & AUROC & FPR95 & AUROC & FPR95 & AUROC & FPR95 & AUROC & FPR95 & AUROC\\

 & $\pmb{\downarrow}$ & $\pmb{\uparrow}$  & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ &  $\pmb{\uparrow}$ & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ \\
\midrule
\emph{Methods using Model Outputs}\\

MSP~\cite{hendrycks2016baseline} & 62.01 & 87.11 & 60.69 & 86.62 & 61.35 & 86.87 & 58.59 & 89.91 & 51.87 & 90.88 & 59.89 & 88.72 & 57.64 & 89.03 &​57.00 & 89.64 \\

ODIN~\cite{liang2018enhancing} & 59.09  & 77.68 & 59.06 & 77.33 & 59.07 & 77.51 & 36.23 & 90.91 & 67.92 & 73.32 & 51.10 & 80.70​& 50.51 & 82.55 & 51.44 & 81.87 \\
GODIN~\cite{hsu2020generalized} & 48.58 & 88.01 & 43.28 & 89.92	& 45.93 & 88.96	& 2.36 & 99.31	& 8.42 & 98.41 & 23.32 & 94.51 & 39.80 & 91.10 & 18.47 & 95.83\\
Energy Score~\cite{liu2020energy} & 51.46 & 86.15 & 45.02 & 88.58 &	48.24 & 87.36 &	44.50 & 90.59 & 44.94 & 88.39 & 48.32 & 86.85 & 41.88 & 89.60 & 44.91 & 88.86 \\
LogitNorm~\cite{wei2022mitigating} & 46.99 & 91.13 & 36.34 & 93.90 & 41.66 & 92.52 & 4.75 & 98.82 &	5.30 & 98.86 & 30.94 & 94.30 & 31.17 & 94.76 & 18.04 & 96.68 \\
DICE~\cite{sun2022dice} & 65.98 & 80.25​& 63.00 & 81.85​& 64.49 & 81.05 & 51.26 & 89.65 &​67.78 & 86.43 & 67.48 & 80.14 &​56.06 & 84.43 &​60.65 & 85.16​ \\
\midrule
\emph{Methods using feature representations}\\
KNN~\cite{sun2022knn} & 52.49 & 89.55 & 46.66 & 91.41​& 49.58 & 90.48 & 50.08 & 91.63 & 33.32 & 95.13 & 46.01 & 92.77 &​43.78 & 91.82 & 43.30 & 92.83​ \\
\midrule
\rowcolor{COLOR_ZS} \name (Ours) & 48.55 & 90.49 & 46.18 & 90.46 & 47.32 & 90.48 & 14.24 & 97.58 & 35.10 & 94.67 & 31.38 & 94.64 & 37.43 & 92.00 & 29.53 & 94.72\\
\bottomrule

\end{tabular}}
\vspace{0.2cm}
\caption{\small Comparison of \name with other competitive baselines on Open-OOD~\cite{yang2022openood} detection benchmark. Results for MSP~\cite{hendrycks2016baseline}, ODIN~\cite{liang2018enhancing}, GODIN~\cite{hsu2020generalized}, Energy~\cite{liu2020energy}, LogitNorm~\cite{wei2022mitigating}, DICE~\cite{sun2022dice}, KNN~\cite{sun2022knn} are directly reported from ~\cite{yang2022openood}. Model is ResNet-18 and ID is CIFAR-10.}
\label{tab:openood_c10}
\end{table}

==> tables/open_ood_c100.tex <==
\begin{table}[t!]

\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l*{6}c|*{10}c}
 \multirow{2}{1.5cm}{\textbf{Methods}} & \multicolumn{6}{c|}{\textbf{Near OOD}} & \multicolumn{10}{c}{\textbf{Far OOD}} \\

\cmidrule{2-17}

& \multicolumn{2}{c}{\textbf{CIFAR-10}} & \multicolumn{2}{c}{\textbf{TIN}} & \multicolumn{2}{c|}{\textbf{Avg.}} &
\multicolumn{2}{c}{\textbf{MNIST}} &
\multicolumn{2}{c}{\textbf{SVHN}} & \multicolumn{2}{c}{\textbf{Textures}} & \multicolumn{2}{c}{\textbf{Places365}} & \multicolumn{2}{c}{\textbf{Avg.}} \\

& FPR95 & AUROC & FPR95 & AUROC & FPR95 & AUROC &  FPR95 & AUROC & FPR95 & AUROC & FPR95 & AUROC & FPR95 & AUROC & FPR95 & AUROC\\

 & $\pmb{\downarrow}$ & $\pmb{\uparrow}$  & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ &  $\pmb{\uparrow}$ & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ & $\pmb{\downarrow}$ & $\pmb{\uparrow}$ \\
\midrule
\emph{Methods using Model Outputs}\\

MSP~\cite{hendrycks2016baseline} & 81.82 & 78.31​& 76.22 & 81.78 &​79.02 & 80.05 & 87.78 & 77.78 & 83.69 & 76.04 & 83.83 & 76.93 & 81.24 & 79.44 & 84.13 & 77.55\\
ODIN~\cite{liang2018enhancing} & 83.16 & 78.18​& 77.77 & 81.39 &​80.46 & 79.79 & 75.34 & 83.71 &​89.76 & 71.08 &​78.37 & 79.39 & 81.27 & 79.83 & 81.18 & 78.50\\
GODIN~\cite{hsu2020generalized} & 85.74 & 71.48 & 76.57 & 81.34 &​81.15 & 76.41 &​48.08 & 91.43 &​71.62 & 86.13 & 58.01 & 88.35 &​78.67 & 78.15​& 64.10 & 86.01​\\
Energy Score~\cite{liu2020energy} & 96.09 & 71.18 & 96.23 & 71.48 & 96.16 & 71.33 & 97.39 & 65.67 & 97.33 & 69.71 & 95.50 & 66.93 & 97.04 & 69.79 &​96.81 & 68.03\\
LogitNorm~\cite{wei2022mitigating} & 83.77 & 74.84 & 77.19 & 81.87 & 86.28 & 78.36 & 53.07 & 90.82 & 79.16 & 83.03 & 87.06 & 71.53 & 80.20 & 79.84 & 74.87 & 81.30\\
DICE~\cite{sun2022dice} &81.91 & 78.50 & 80.87 & 80.72 & 81.39 & 79.61 & 81.68 & 78.02 & 79.93 & 79.97 & 80.53 & 77.70 & 80.75 & 80.18 & 80.72 & 78.97  \\
\midrule
\emph{Methods using feature representations}\\
KNN~\cite{sun2022knn} & 82.11 & 76.52 & 73.78 & 83.35 & 77.94 & 79.94 & 79.08 & 83.80 & 74.27 & 82.21 & 66.40 & 83.81 &	78.74 & 79.10 & 74.62 & 82.23\\
\midrule
\rowcolor{COLOR_ZS} \name (Ours) & 81.98 & 74.65 & 74.75 & 80.23 & 78.36 & 77.44 & 52.61 & 88.27 & 54.20 & 86.83 & 79.83 & 75.34 & 75.40 & 78.31 & 65.57 & 82.13\\
\bottomrule

\end{tabular}}
\vspace{0.2cm}
\caption{\small Comparison of \name with other competitive baselines on Open-OOD~\cite{yang2022openood} detection benchmark. Results for MSP~\cite{hendrycks2016baseline}, ODIN~\cite{liang2018enhancing}, GODIN~\cite{hsu2020generalized}, Energy~\cite{liu2020energy}, LogitNorm~\cite{wei2022mitigating}, DICE~\cite{sun2022dice}, KNN~\cite{sun2022knn} are directly reported from ~\cite{yang2022openood}. Model is ResNet-18 and ID is CIFAR-100.}
\label{tab:openood_c100}
\end{table}

==> tables/train_time.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\small
\centering
\caption{\small Performance comparison on CIFAR-100 dataset for various network architectures. All values are averaged over multiple OOD test datasets. Best results are in \textbf{bold}.}
\label{tab:arch}
\begin{tabular}{lcccc}
\textbf{Method} & \textbf{Architecture} & \textbf{FPR95}  & \textbf{AUROC} \\ 
& & $\downarrow$ & $\uparrow$ \\ 
\toprule
KNN~\cite{sun2022knn} & DenseNet-101 & 47.21 & 85.27 \\ 
 \name (ours) & DenseNet-101 &  \textbf{31.25} &  \textbf{90.76}\\ 
\midrule
KNN~\cite{sun2022knn} & ResNet-50 & 53.05 & 83.61 \\ 
\name (ours) & ResNet-50 &  \textbf{45.51} & \textbf{86.81} \\ 
\bottomrule
\end{tabular}
\vspace{-0.4cm}
\end{wraptable}


==> tables/vit_ood.tex <==
\newcolumntype{?}{!{\vrule width 1pt}}
\begin{table}[h]
\centering
\small
\begin{tabular}{l*{4}c}
\toprule
\multirow{2}{1.5cm}{\textbf{Methods}} & \multicolumn{3}{c}{\textbf{OOD Datasets}} & \multirow{2}{*}{\textbf{ID Acc.}} \\

\cmidrule{2-4}


& \textbf{C-10} & \textbf{SVHN} & \textbf{Places-365} & \\
 \midrule
KNN~\cite{sun2022knn} &  \\
\rowcolor{COLOR_ZS} \name (ours) & \\

\bottomrule

\end{tabular}
\caption{Performance comparison (FPR95) on ViT-B/16 model fine-tuned on CIFAR-100 dataset.}
\label{tab:vit_ood}
\end{table}


